Computing Maxmin Strategies in Extensive-Form Zero-Sum Games with Imperfect Recall

Extensive-form games with imperfect recall are an important game-theoretic model that allows a compact representation of strategies in dynamic strategic interactions. Practical use of imperfect recall games is limited due to negative theoretical results: a Nash equilibrium does not have to exist, computing maxmin strategies is NP-hard, and they may require irrational numbers. We present the first algorithm for approximating maxmin strategies in two-player zero-sum imperfect recall games without absentmindedness. We modify the well-known sequence-form linear program to model strategies in imperfect recall games and use a recent technique to approximate bilinear terms. Our main algorithm is a branch-and-bound search over these linear programs that provably reaches a desired approximation after an exponential number of steps in the size of the game. Experimental evaluation shows that the proposed algorithm can approximate maxmin strategies of randomly generated imperfect recall games of sizes beyond toy-problems within few minutes.

==> intro.tex <==
\section{Introduction}
We focus on computing strategies in two-player zero-sum \emph{extensive-form games} with partial observability and stochastic events (EFGs).

The main characteristic of EFGs that affects the computational complexity of finding optimal strategies is the notion of \emph{perfect recall}.
In games with perfect recall, players remember all their previously played moves and all information gathered during the game. The  \emph{imperfect recall} games relax this assumption. The imperfect recall games can be further restricted to A.loss recall games~\cite{kaneko1995,kline2002}, where every loss of information of a player can be tracked to a loss of informqation about his own action.
%It is well known that in games with perfect recall a Nash equilibrium (NE) in behavioral strategies always exists~\cite{Kuhn1953}.
%Moreover, computing a NE in EFGs with perfect recall is a polynomial problem~\cite{Koller1996,vonStengel96}.

%This is not true for games with \emph{imperfect recall}. % that introduce new challenges compared to perfect recall games.
In imperfect recall games a Nash equilibrium (NE) in behavioral strategies does not have to exist~(e.g., see Figure~\ref{fig:example}), and deciding whether a NE exists is an NP-hard problem~\cite{miltersen2007}.
As an alternative, we can seek a strategy maximizing the guaranteed expected outcome of a game, \emph{a maxmin strategy}, which always exists.
Maxmin strategies may require irrational numbers even when the input uses rational numbers~\cite{koller1992}.
So finding optimal strategies has fundamental difficulties, and approximating maxmin strategies is equivalent to solving imperfect recall games. %, hence, we cannot have an exact algorithm using a standard a. And so, approximating maxmin strategies is equivalent to solving imperfect recall games.
Deciding whether a player with imperfect recall can guarantee a given value in an imperfect recall game is, however, an NP-hard problem~\cite{koller1992}.

%Despite the negative theoretical results, imperfect recall games appear in practical equilibrium computation~\cite{waugh2009practical,lanctot2012}. 
%Methods for solving large perfect recall games often use abstractions (such as merging certain information sets together) that can lead to imperfect recall games~\cite{gilpin2007,kroer2014extensive,kroer2014extensiveIR}.
%Moreover, since the imperfect recall games in these cases are the result of an abstraction method, one can decide about the choices made by the abstraction algorithm such that only imperfect recall games with desired properties are created. 
%An example is the poker domain, where one can create so called \emph{(skewed) well-formed games} in which the standard perfect-recall algorithms (namely Counterfactual Regret Minimization; CFR) are still guaranteed to find an approximate Nash (no-regret) behavioral strategy~\cite{lanctot2012,kroer2014extensiveIR}.
%However, the restrictions on games to form a well-formed game are rather strict and the perfect-recall algorithms fail when there is no NE in behavioral strategies.
%If the games do not satisfy these restrictions there is, to the best of our knowledge, no practical algorithm for computing maxmin strategies in imperfect recall games.

We propose the first algorithm for approximating maxmin behavioral strategies in imperfect recall games with no \emph{absentmindedness}, where each decision point in the game is visited at most once during the course of the game. This is arguably a natural restriction in finite games (see, e.g., \cite{piccione1997}). 
Our approach extends the sequence-form linear program~\cite{koller1996,vonStengel96} with additional bilinear constraints necessary for the correct representation of strategies in imperfect recall games.
We approximate bilinear terms using Multiparametric Disaggregation Technique (MDT) due to~\cite{Kolodziej2013}, obtaining mixed-integer linear programs (MILP) for computing lower and upper bounds on the expected maxmin value of player 1. % with size linear to the size of the game.
Next, we use the linear program (LP) relaxation of the MILP for computing upper bounds to design the main branch-and-bound algorithm, which repeatedly solves the relaxed LP and tightens constraints for imperfect recall and relaxed binary variables from the MILP. Finally we bound the number of iterations needed by the branch-and-bound algorithm to find an $\epsilon$-optimal solution.

%Given our motivation that imperfect recall games can be created using abstraction methods from perfect recall games, one can control some properties of imperfect recall in the abstracted game.
We propose two variants of our algorithm depending on the type of recall of player 2: (1) we assume player 2 has  A-loss recall, or (2) the only restriction on the imperfect recall of player 2 is no absentmindedness (the only restriction for player 1 is no absentmindedness in both cases). %The second version of the algorithm is presented in the appendix.%Due to the space constraints, we describe the case with the local best response in the appendix.
%To demonstrate the performance of our algorithm, we provide a short experimental evaluation and show that it can solve games of sizes far beyond toy problems (up to $4 \cdot 10^4$ states) typically within a few minutes. 
%The first algorithm can solve games of sizes far beyond toy problems (up to $4 \cdot 10^4$ states) typically within a few minutes.
Due to the space constraints, the second version of the algorithm, as well as all proofs are in the appendix.
%All the proofs are presented in the appendix, due to space constraints. 

%The paper is structured as follows.
%We first provide necessary technical background on extensive-form games, imperfect recall, and we explain the original methods that we use in our approach (the sequence form and MDT discretization technique).
%Next we incrementally explain our novel algorithm.
%We give the bilinear sequence form, following by the mixed-integer (MILP) approximations of the bilinear program for computing lower and upper bounds, and we formally prove error bounds for these programs. 
%%The theoretical analysis identifies variables that contribute to the error of MILPs.
%%We exploit this information in the main algorithm. 
%Then we propose our main branch-and-bound algorithm that uses a relaxation of all binary variables of the upper-bound MILP and that iteratively tightens both types of error -- one due to the MDT discretization and the second one due to the relaxation of binary variables.
%Finally, we provide a short experimental evaluation to demonstrate the practical scalability of our algorithm and show that it is indeed a practical algorithm that can solve games of sizes far beyond toy problems (up to $4 \cdot 10^5$ states) typically in few minutes. 


